Galaxy Assembly and Evolution in the P-Millennium simulation: galaxy clustering

[abridged] We present results from the latest version of the GAEA theoretical model of galaxy formation coupled with merger trees extracted from the Planck Millennium Simulation (PMS). With respect to the Millennium Simulation, the PMS provides a better mass resolution, a larger volume and assumes cosmological parameters consistent with latest results from the Planck mission. The model includes a treatment for the partition of cold gas into atomic and molecular (H$_2$) components; a better treatment for environmental processes; an updated modelling of cold gas accretion on Super-Massive Black Holes. We compare GAEA predictions based on the PMS, with model realizations based on other simulations in the Millennium Suite, showing that the new model provides a remarkable consistency for most statistical properties of galaxy populations. We interpret this as due to the interplay between AGN feedback and H$_2$-based SFR, as model versions considering only one of the two mechanisms do not show the same level of consistency. We then compare model predictions with available data for the galaxy 2-point correlation function (2pCF) in the redshift range 0<z$\lesssim$3. We show that GAEA runs correctly recover the main dependencies of the 2pCF as a function of stellar mass, star formation activity, HI-content and redshift for galaxies more massive than 10$^{9}$ M$_\odot$. These results suggest that our model correctly captures both the distribution of galaxy populations in the Large Scale Structure and the interplay between the main physical processes regulating their baryonic content, both for central and satellite galaxies. The model predicts a small redshift evolution of the clustering amplitude, that results in an overprediction of z$\sim$3 clustering strength with respect to the available estimates, but is still consistent with data within 1-$\sigma$ uncertainties.

==> journal.tex <==
%%%%%%%%% Bibliography and bibfile
\def\aj{AJ}%
         % Astronomical Journal
\def\araa{ARA\&A}%
         % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
         % Astrophysical Journal
\def\apjl{ApJ}%
         % Astrophysical Journal, Letters
\def\apjs{ApJS}%
         % Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}%
         % Applied Optics
\def\apss{Ap\&SS}%
         % Astrophysics and Space Science
\def\aap{A\&A}%
         % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
         % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
         % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
         % Astronomicheskii Zhurnal
\def\baas{BAAS}%
         % Bulletin of the AAS
\def\jrasc{JRASC}%
         % Journal of the RAS of Canada
\def\memras{MmRAS}%
         % Memoirs of the RAS
\def\mnras{MNRAS}%
         % Monthly Notices of the RAS
\def\pra{Phys.~Rev.~A}%
         % Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}%
         % Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}%
         % Physical Review C
\def\prd{Phys.~Rev.~D}%
         % Physical Review D
\def\pre{Phys.~Rev.~E}%
         % Physical Review E
\def\prl{Phys.~Rev.~Lett.}%
         % Physical Review Letters
\def\pasp{PASP}%
         % Publications of the ASP
\def\pasj{PASJ}%
         % Publications of the ASJ
\def\qjras{QJRAS}%
         % Quarterly Journal of the RAS
\def\skytel{S\&T}%
         % Sky and Telescope
\def\solphys{Sol.~Phys.}%
         % Solar Physics
\def\sovast{Soviet~Ast.}%
         % Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}%
         % Space Science Reviews
\def\zap{ZAp}%
         % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
         % Nature
\def\iaucirc{IAU~Circ.}%
         % IAU Cirulars
\def\aplett{Astrophys.~Lett.}%
         % Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}%
         % Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}%
         % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}%
         % Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}%
         % Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}%
         % Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}%
         % Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}%
         % Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
         % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}%
         % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}%
         % Nuclear Physics A
\def\physrep{Phys.~Rep.}%
         % Physics Reports
\def\physscr{Phys.~Scr}%
         % Physica Scripta
\def\planss{Planet.~Space~Sci.}%
         % Planetary Space Science
\def\procspie{Proc.~SPIE}%
         % Proceedings of the SPIE
\def\nar{NewAR}%
         % New Astronomy Review?
\def\na{NewA}%
         % New Astronomy ?
\def\jcap{JCAP}%
         % Journal of Cosmology and Astroparticle Physics?
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

